HULK-V: a Heterogeneous Ultra-low-power Linux capable RISC-V SoC

IoT applications span a wide range in performance and memory footprint, under tight cost and power constraints. High-end applications rely on power-hungry Systems-on-Chip (SoCs) featuring powerful processors, large LPDDR/DDR3/4/5 memories, and supporting full-fledged Operating Systems (OS). On the contrary, low-end applications typically rely on Ultra-Low-Power ucontrollers with a "close to metal" software environment and simple micro-kernel-based runtimes. Emerging applications and trends of IoT require the "best of both worlds": cheap and low-power SoC systems with a well-known and agile software environment based on full-fledged OS (e.g., Linux), coupled with extreme energy efficiency and parallel digital signal processing capabilities. We present HULK-V: an open-source Heterogeneous Linux-capable RISC-V-based SoC coupling a 64-bit RISC-V processor with an 8-core Programmable Multi-Core Accelerator (PMCA), delivering up to 13.8 GOps, up to 157 GOps/W and accelerating the execution of complex DSP and ML tasks by up to 112x over the host processor. HULK-V leverages a lightweight, fully digital memory hierarchy based on HyperRAM IoT DRAM that exposes up to 512 MB of DRAM memory to the host CPU. Featuring HyperRAMs, HULK-V doubles the energy efficiency without significant performance loss compared to featuring power-hungry LPDDR memories, requiring expensive and large mixed-signal PHYs. HULK-V, implemented in Global Foundries 22nm FDX technology, is a fully digital ultra-low-cost SoC running a 64-bit Linux software stack with OpenMP host-to-PMCA offload within a power envelope of just 250 mW.

==> TEXT/SW_LV.tex <==
\section{Software Stack and Programming Model}\label{Softwarestack}
\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{images/sw_stack.pdf} 
    \caption{HULK-V software stack (from hardware to user-space)}
    \label{fig:openMP}
    \vspace{-4mm}%Put here to reduce too much white space after your table
\end{figure}
HULK-V comes with a mature software stack for heterogeneous programming, as illustrated in Figure~\ref{fig:openMP}.
It includes a full-fledged Buildroot-based Linux (v5.16.9) distribution running on the CVA6 host processor, featured by a complete heterogeneous programming model based on Clang/LLMV 12 OpenMP 5 for efficiently offloading and programming the PMCA cluster.
The HULK's software stack furnishes a well-known, popular, and mainstream set of user-level libraries, easing the programmability and enabling straightforward porting of legacy Linux-compatible applications.

CVA6's MMU supports SV39 virtual memory paging~\cite{privilegedriscv}, while the PMCA can only generate 32-bit addresses. A special shared region in the main memory, accessible through user-space \emph{hulk\_malloc()} function, enables data sharing in this mixed-address space. The function allocates contiguous memory buffers within accessible memory space, making the pointer sharing between the subsystems straightforward.

PMCA cluster exposes a Linux Driver and user-space API to the CVA6 for loading and executing programs both through lightweight bare-metal programming and high-level OpenMP 5 heterogeneous programming.

Bare-metal programming allows low overheads and fine-grained access to the hardware on PMCA, and it is mainly used for functional validation, performance assessment and power profiling. 

However, one must write two different codes for the host and cluster. To avoid this, HULK-V adopted the OpenMP 5 framework from HERO~\cite{herov2}, allowing users to use a high-level, directive-based, intuitive programming interface to efficiently offload the computationally intensive part of a program to the PMCA within one single heterogeneous source code.

The HULK-V software stack comes with runtime libraries and compiler extensions of the Clang/LLVM 12 compiler for OpenMP 5 offload support from CVA6 ISA to RI5CY ISA. HULK-V is the first 100\% RISC-V instance of HERO.

==> TEXT/SW_YT.tex <==
\section{Software Stack and Programming Model}\label{Softwarestack}
\begin{figure}
    \centering
    \includegraphics[width=.5\textwidth]{images/sw_stack.pdf}
    \caption{HULK-V software stack (from hardware to user-space)}
    \label{fig:openMP}
    \vspace{-4mm}%Put here to reduce too much white space after your table 
\end{figure}
HULK-V’s software stack is illustrated in Figure \ref{fig:openMP} and has been extensively validated on the FPGA-emulated HULK-V. Thanks to Linux and OpenMP support, HULK-V provides the most popular and mainstream set of user-level libraries, easing the programmability and enabling straightforward porting of any Linux-compatible application.

On the PMCA side, HULK-V supports a lightweight bare-metal runtime that allows low programming overhead and is optimized for the small L1SPM. The PMCA runtime also allows hardware functionality validation and performance and power profiling. On the host side, CVA6 runs a full-fledged Buildroot-based Linux distribution equipped with a dedicated driver for the PMCA management but also supports a HULK-
V bare-metal runtime.

The APIs provided by the PMCA runtime and the Linux driver are already sufficient to run heterogeneous code on the platform. However, one must write the host and cluster code separately. To avoid this, we adapted to HULK-V the OpenMP framework from HERO\cite{herov2}, providing the software developers with an intuitive programming interface to easily declare the kernels to be offloaded on the PMCA within one single heterogeneous source code.

To support OpenMP, we adapted an extended version of the LLVM/Clang 12 compiler porting it from the CortexA53 host to CVA6, making HULK-V the first 100\% RISC-V instance of HERO. OpenMP generates one unified heterogeneous binary for both host and target (the PMCA), automatically invoking the PMCA and the PMCA-Linux APIs.

Regarding virtual memory, CVA6’s MMU supports SV39\cite{privilegedriscv} virtual memory paging, while the PMCA can only generate 32-bit addresses. Data sharing is enabled by labeling a portion of the main L3 memory as a shared memory region. This way the host generates data for the cluster by calling a custom \textit{hulk malloc()} function, allocating the data in the shared buffer and returning the physical address of the allocated region. Pointer sharing is straightforward when virtual memory is not enabled.
